The Almost Equivalence by Asymptotic Probabilities for Regular Languages and Its Computational Complexities

We introduce p-equivalence by asymptotic probabilities, which is a weak almost-equivalence based on zero-one laws in finite model theory. In this paper, we consider the computational complexities of p-equivalence problems for regular languages and provide the following details. First, we give an robustness of p-equivalence and a logical characterization for p-equivalence. The characterization is useful to generate some algorithms for p-equivalence problems by coupling with standard results from descriptive complexity. Second, we give the computational complexities for the p-equivalence problems by the logical characterization. The computational complexities are the same as for the (fully) equivalence problems. Finally, we apply the proofs for p-equivalence to some generalized equivalences.

==> eptcsdata.tex <==
\providecommand{\firstpage}{272}
\providecommand{\publicationstatus}{D. Cantone and G. Delzanno (Eds.): Seventh Symposium on\\
Games, Automata, Logics and Formal Verification (GandALF'16)\\
EPTCS 226, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.226.19}{10.4204/EPTCS.226.19}}

